A High-Level Comparison of Recent Technologies for Massive MIMO Architectures

Since the introduction of massive MIMO (mMIMO), the design of a transceiver with feasible complexity has been a challenging problem. Initially, it was believed that the main issue in this respect is the overall RF-cost. However, as mMIMO is becoming more and more a key technology for future wireless networks, it is realized, that the RF-cost is only one of many implementational challenges and design trade-offs. In this paper, we present, analyze and compare various novel mMIMO architectures, considering recent emerging technologies such as intelligent surface-assisted and Rotman lens based architectures. These are compared to the conventional fully digital (FD) and hybrid analog-digital beamforming (HADB) approaches. To enable a fair comparison, we account for various hardware imperfections and losses and utilize a novel, universal algorithm for signal precoding. Based on our thorough investigations, we draw a generic efficiency to quality trade-off for various mMIMO architectures. We find that in a typical cellular communication setting the reflect/transmit array based architectures sketch the best overall trade-off. Further, we show that in a qualitative ranking the power efficiency of the considered architectures is independent of the frequency range.

==> capacity_cost.tex <==
\begin{tikzpicture}
	\begin{axis}[
		axis lines = left,
		xlabel = Number of antennas,%/\ac{rf} chains,
		%ylabel = {\color{blue}Capacity}/{\color{orange}Cost},
		%xticklabels = {$N_\mathrm{e}$},
		%xtick = {3},
		xtick=\empty,
		%yticklabels = {},
		ytick = \empty,
		]
		\addplot[
		domain = 0.1:6, 
		samples = 500,
		color = orange,
		line width = 1.5pt,
		]
		{1.5*x} node at (axis cs:2.6,6) {\color{orange} \bfseries Complexity/};
		\addplot[
		domain = 0.1:6, 
		samples = 500,
		color = orange,
		line width = 1.5pt,
		]
		{1.5*x} node at (axis cs:2.6,5.4) {\color{orange} \bfseries Cost};
		]
		\addplot[
		domain = 0.1:6,
		samples = 500,
		color = blue,
		line width = 1.5pt,
		]
		%{ln(x)/ln(2)};
		%Rapp model
		{1.5*x/( (1+ (abs(1.5*x)/5)^3 ) )^(1/3)} node at (axis cs:3.8,3) {\color{blue} \bfseries Capacity};
		%log
		%{ln(x)/ln(1.4)} node at (axis cs:3.8,3.5) {\color{blue} \bfseries Capacity};
	\end{axis}
\end{tikzpicture}
